Benchmarking Quantum Annealers with Near-Optimal Minor-Embedded Instances

Benchmarking Quantum Process Units (QPU) at an application level usually requires considering the whole programming stack of the quantum computer. One critical task is the minor-embedding (resp. transpilation) step, which involves space-time overheads for annealing-based (resp. gate-based) quantum computers. This paper establishes a new protocol to generate graph instances with their associated near-optimal minor-embedding mappings to D-Wave Quantum Annealers (QA). This set of favorable mappings is used to generate a wide diversity of optimization problem instances. We use this method to benchmark QA on large instances of unconstrained and constrained optimization problems and compare the performance of the QPU with efficient classical solvers. The benchmark aims to evaluate and quantify the key characteristics of instances that could benefit from the use of a quantum computer. In this context, existing QA seem best suited for unconstrained problems on instances with densities less than $10\%$. For constrained problems, the penalty terms used to encode the hard constraints restrict the performance of QA and suggest that these QPU will be less efficient on these problems of comparable size.

==> outline.tex <==
\section{Publication outline}

Tight Analysis of Quantum Optimization Systems: a new method to explore the performance of optimization problems based on graphs. The aim is to study the scaling of graph optimization problems on quantum computers using near-optimal embedding strategies.

\noindent
\textbf{Motivations:}
\begin{itemize}
    \item Mapping graph problems on quantum chips using NISQ devices require either Swapping network (for Quantum circuits) or Minor-embeddding techniques (for QA).
    \item Quadratic increase in the number of qubits on fixed topology Quantum Annealers. Linear increase for quantum circuits. Leads to exponential increase of noise due to quantum noise.
    \item The aim is to study the performance of the quantum systems with near-optimal embedding techniques. (Experiments done on D-Wave QC)
\end{itemize}


\noindent
\textbf{Introduction}
\begin{itemize}
    \item Application-oriented benchmarks (graph optimization framework).
    \item Overhead of SWAP / number of qubits have a negative impact on the resolution of quantum problems.
    \item Contributions: Proposition of a classification of graph problems mapping hardness. Analysis of the performance of Quantum Annealers on problems of a gradual "friendliness". Density scaling threshold.
\end{itemize}

\noindent
\textbf{Related work}
\begin{itemize}
    \item Méthodes de benchmark: Citer "Defining and detecting quantum speedup" (ising problem study), citer "Demonstration of a scaling advantage for a quantum annealer over simulated annealing".
    \item Introduce minor embedding methods
    \item Introduce the different metrics required for benchmarks: quality, speed, cost (i.e. energy / Total cost of ownership etc.)
    \item Introduce common benchmark approaches (classification of existing methods ?)
\end{itemize}

\noindent
\textbf{Classication of Graph problems}
\begin{itemize}
    \item Identify the requirements of each graph problem.
    \item Presentation of the parameters used for the classification. (Encoding of constraints, e.g. Hadfield implementation of the MIS).
\end{itemize}


\noindent
\textbf{Method}
\begin{itemize}
    \item Focus on the metrics (minor-embedding quality, $\epsilon$-close metric introduced in TAQOS)
    \item Focus on the method used for instance generation using edge contraction (possibility to do the same with quantum circuits and swapping networks)
    \item Problem instances generated: Max-cut problems, High precision Ising model with different weight distributions, MIS, Knapsack, TSP, others ?
    \item Instance space analysis using TAQOS
\end{itemize}

List of graph problems from Karp (Formulation QUBO):
\begin{itemize}
    \item Max-cut (coded)
    \item Weighted Max-cut (coded)
    \item Clique (MAX-clique $\equiv$ MIS on complementary graph $G'(V,E')$ of $G(V,E)$ : $E' = \{(u,v) \forall (u,v) \notin E\}$ 
    \item Clique cover
    \item Vertex Cover (coded, max -f, f for MIS)  
    \item Set covering
    \item Feedback arc set
    \item Feedback vertex set
    \item Coloration
    \item MIS (coded)
    \item TSP (Hamiltonian circuit)
    \item Knapsack (coded)
    \item Job sequencing
    \item 3-D Matching
    \item Steiner tree
\end{itemize}

\noindent
D-Wave parameter settings (default parameter): uniform weight spreading, chain strength obtained with \textit{uniform\_torque\_compensation}, majority vote at the end of the annealing process. ($815$ shots at $1000 \mu s$ each)

\noindent
D-Wave parameter settings (optimized parameters): uniform weight spreading, chain strength obtained with binary search (add a local scan ?), majority vote at the end, Spin reversal added, annealing offsets added.

\noindent
\textbf{Results}
\begin{itemize}
    \item Analysis of the performance of QA default behavior. Near-optimal mapping, default torque compensation, uniform weight spreading, auto-scale, default annealing offset, post-processing with majority vote.
    \item Analysis of the performance of QA optimized behavior. Combining SR, Annealing offsets and optimal chain strength. Unveil optimal pre-processing time required (using TAQOS library).
    \item Reverse instance feature analysis using TAQOS.
\end{itemize}

\noindent
\textbf{Conclusion}
\begin{itemize}
    \item Conclude on the performance analysis
    \item Give some clues to extend this approach to Quantum Circuit.
    \item Compare out results with QUBO-Plus (Heuristic designed to handle specific types of constraints). See paper of Glover "Quantum Bridge Analytics II: QUBO-Plus, network optimization and combinatorial chaining for asset exchange"
    \item It could be interesting to develop a classical heuristic that take advantage of instances structure that are near the D-Wave structure to see if the advantage of D-Wave persist.  
\end{itemize}



\textbf{Classify sets of problems according to their difficulty:}
Split optimization problem between constrained and unconstrained
Criteria of the classification: is constrained, constraint relaxation method (e.g. penalty),   
\begin{itemize}
    \item Unweighted perfect (compare QA with Simulated Annealing). Maxcut-problem
    \item Weighted perfect (spin glass problem with $J_{ij}$ Gaussianly sampled). (weighted max-cut). Find problem with weighted $h_i$
    \item Unweighted with topology mapping requirements. (max-cut problems)
    \item Weighted with topology mapping requirements. (Weighted max-cut, MIS, Vertex color etc.)
    \item Fully connected problems (unweighted as SK-model)
    \item Fully connected weighted (Knapsak problem, graph partitionning, graph coloring, TSP ...)
    \item Higher order binary optimization problems, which require qubo transformation (such as QAP, Hypergraph partitioning)
\end{itemize}

The difficulty of the instance is closely related to the hardware architecture. Classify existing optimization problem in this set of difficulty.


